TransTIC: Transferring Transformer-based Image Compression from Human Perception to Machine Perception

This work aims for transferring a Transformer-based image compression codec from human perception to machine perception without fine-tuning the codec. We propose a transferable Transformer-based image compression framework, termed TransTIC. Inspired by visual prompt tuning, TransTIC adopts an instance-specific prompt generator to inject instance-specific prompts to the encoder and task-specific prompts to the decoder. Extensive experiments show that our proposed method is capable of transferring the base codec to various machine tasks and outperforms the competing methods significantly. To our best knowledge, this work is the first attempt to utilize prompting on the low-level image compression task.

==> Figures/Ablation_STBs_1.tex <==
\begin{figure}[t]
\centering
\subfigure[Classification]{
\centering
\includegraphics[width=0.49\linewidth]{Figures/RD-curve/Imagenet_cls_rdaccuracy_ablation2.png}
}
\hspace{-0.35cm}
\subfigure[Object Detection]{
\centering
\includegraphics[width=0.49\linewidth]{Figures/RD-curve/MSCOCO_det_rdmap_ablation2.png}
}
\caption{Ablation on IP-type and TP-type STBs.}
\label{fig:STB_ablation}
\end{figure}

==> Figures/Ablation_prompts_1.tex <==
\begin{figure}[t]
\centering
\subfigure[Classification]{
\centering
\includegraphics[width=0.49\linewidth]{Figures/RD-curve/Imagenet_cls_rdaccuracy_ablation1.png}
}
\hspace{-0.35cm}
\subfigure[Object Detection]{
\centering
\includegraphics[width=0.49\linewidth]{Figures/RD-curve/MSCOCO_det_rdmap_ablation1.png}
}
\caption{Ablation on the depth and number of prompts.}
\label{fig:prompts_ablation}
\end{figure}

==> Figures/RD_curves_ablation.tex <==
\begin{figure*}[t]
\centering
\subfigure[Classification]{
\centering
\includegraphics[width=0.235\linewidth]{Figures/RD-curve/Imagenet_cls_rdaccuracy_ablation2.png}
}
\subfigure[Object Detection]{
\centering
\includegraphics[width=0.235\linewidth]{Figures/RD-curve/MSCOCO_det_rdmap_ablation2.png}
}
\subfigure[Classification2]{
\centering
\includegraphics[width=0.235\linewidth]{Figures/RD-curve/Imagenet_cls_rdaccuracy_ablation1.png}
}
\subfigure[Object Detection2]{
\centering
\includegraphics[width=0.235\linewidth]{Figures/RD-curve/MSCOCO_det_rdmap_ablation1.png}
}
\caption{}
\label{fig:RD_ablation}
\end{figure*}

==> Figures/STB.tex <==
\begin{figure*}[t]
\centering
\subfigure[]{
\centering
\includegraphics[scale=0.13,trim=0 0 1620 0,clip]{Figures/STB.png}
}
\subfigure[]{
\centering
\includegraphics[scale=0.13,trim=1950 0 0 0,clip]{Figures/STB.png}
}
\caption{}
\label{fig:STB}
\end{figure*}


==> Figures/mpeg_1.tex <==
\begin{figure}[t]
\centering
\subfigure{
    \centering
    \includegraphics[width=.3\textwidth]{Figures/mpeg/OpenImage_det_fin.png}
    \label{fig:rd-a}
    }
\subfigure{
    \centering
    \includegraphics[width=.3\textwidth]{Figures/mpeg/OpenImage_seg_fin.png}
    \label{fig:rd-b}
}
\caption{Rate-mAP comparison against MPEG VCM proposals.}
\label{fig:MPEG}
\vspace{-0.2cm}
\end{figure}

==> Sections/Complexity.tex <==
\input{Tables/complexity}
\section{Complexity Comparison}
\label{sec:complexity}
Table~\ref{tab:complexity} compares the complexity of the competing methods in terms of the kilo-multiply-accumulate-operations per pixel (kMACs/pixel) and model size. Through transferring the pre-trained \textit{TIC}, our \textit{TransTIC} only needs to learn for each task a prompt generation network on the encoder side and several task-specific prompts on the decoder side. The number of these additional parameters is about one fifth of that of a complete \textit{TIC} (7M). %It is notably lower than training a complete, separate \textit{TIC} (7M) with \textit{full fine-tuning} for each task. 
As compared with \textit{TIC}, the increase in kMACs/pixel (i.e. from 188 to 202) on the decoder side is modest. In contrast, our~\textit{TransTIC} has a much more complex encoder than~\textit{TIC} because of incorporating a prompt generation network, which must adapt the encoder-side prompts to the downstream task and the current input image. Nevertheless, \textit{TransTIC} offers significantly lower kMACs/pixel and parameters than ROI~\cite{ICCV21} and \textit{TIC+SFT}~\cite{wang2018sftgan}, both of which utilize more computationally heavy networks for SFT layers. Furthermore, ROI~\cite{ICCV21} currently uses a pre-trained recognition network to generate the ROI mask. This results in much higher kMACs/pixel on the encoder side. Table~\ref{tab:complexity} provides the kMACs/pixel needed to generate the ROI masks for different tasks. Last but not least, \textit{TIC+channel selection}~\cite{channelselection} has a low-complexity decoder (which is composed of only the hyperprior decoder and the transform module) because it need not reconstruct the input image. However, it performs much worse than our~\textit{TransTIC} (see Fig.~3 in the main paper).


%doesn't reconstruct the image, its performance is evidently inferior to all other methods.
% It is notably lower than training a complete, separate \textit{TIC} (7M) with \textit{full fine-tuning} for each task.
% \input{Tables/complexity}


==> Sections/Generalization.tex <==
\section{Generalization}
\label{generalization}


==> Sections/MPEG.tex <==
\section{Comparison with MPEG VCM Proposals}
\label{sec:mpeg}
\textcolor{red}{In this section, we compare our TransTIC with the methods recently submitted to the call-for-proposals (CFP) competition of the MPEG VCM standard based on their test protocol\cite{MPEGVCMctc}. The results of these competing methods are from the CFP test report~\cite{MPEGm61010}. As shown in Fig.~\ref{fig:MPEG}, our TransTIC performs comparably to the top performers in terms of rate-accuracy performance. However, our base codec has the additional constraint that it is optimized for human perception, while the top performers (e.g. p12, p6, p7) optimize the entire codec end-to-end for machine tasks. This shows the potential of our TransTIC.}

\input{Figures/mpeg}


==> Tables/complexity_1.tex <==
\begin{table}[]
\centering
\caption{Comparison of the kMACs/pixel and model size.}
\setlength{\tabcolsep}{4.0pt}
\fontsize{8}{8}\selectfont
\begin{tabular}{cc|cc|cc}
\toprule
\multicolumn{2}{l|}{}                                                                             & \multicolumn{2}{c|}{\textbf{kMACs/pixel}} & \multicolumn{2}{c}{\textbf{Params (M)}} \\
\multicolumn{2}{l|}{}                                                                             & Encoder         & Decoder        & Encoder            & Decoder            \\ \midrule 
\multicolumn{2}{c|}{\textit{TIC}}                                                                 & 142.54          & 188.52         & 3.65               & 3.86               \\ \midrule 
\multicolumn{1}{c}{\multirow{4}{*}{ROI~\cite{ICCV21}}}  & Autoencoder only  & 800.36          & 679.80         & 21.91              & 5.65               \\
\multicolumn{1}{c}{}                                                          & Classification    & 882.46          & 679.80         & 47.47              & 5.65               \\
\multicolumn{1}{c}{}                                                          & Detection         & 991.13          & 679.80         & 63.39              & 5.65               \\
\multicolumn{1}{c}{}                                                          & Segmentation      & $\approx$997.85          & 679.80         & 66.03              & 5.65               \\ \midrule 
\multicolumn{2}{c|}{\textit{TIC+SFT}~\cite{wang2018sftgan}}                & 686.39          & 462.23         & 12.08              & 9.62               \\
\multicolumn{2}{c|}{\textit{TIC+channel selection}~\cite{channelselection}} & 142.54          & 25.13          & 3.76               & 1.96               \\
\multicolumn{2}{c|}{Ours (\textit{TransTIC})}                                                  & 332.03          & 202.60         & 5.24               & 3.89               \\  
\bottomrule
\end{tabular}
\label{tab:complexity}
\end{table}

==> Tables/content_vs._task.tex <==
\begin{table}[]
\caption{Ablation of introducing instance-specific vs. task-specific on the encoder side.}
\fontsize{8}{8}\selectfont
\centering
\begin{tabular}{c|c|c}
\toprule
                 & Instance-specific & Task-specific \\
\midrule
Classification   &  -56.6  &  -42.9   \\
Object Detection &  \textcolor{red}{-51.9}  &  -32.6   \\
\bottomrule
\end{tabular}
\label{tab:content_vs_task}
\end{table}

==> Tables/decoder_side.tex <==
\begin{table}[]
\caption{Ablation of task-specific prompts at the decoder side.}
\fontsize{8}{8}\selectfont
\centering
\begin{tabular}{c|c|c}
\toprule
                 & Task-specific prompts & No prompts \\
\midrule
Classification   &  -56.6  &  -49.7   \\
Object Detection &  \textcolor{red}{-51.9}  &  \textcolor{red}{-28.3}   \\
\bottomrule
\end{tabular}
\label{tab:decoderside}
\end{table}

==> Tables/generalization_cls.tex <==
\begin{table}[]
\caption{Analysis on generalization ability of different methods. All methods are trained on ResNet50, then tested on ResNet50 and VGG19 respectively. The BD-rate shown are computed with \textit{Swin} tesed on ResNet50 and VGG19 as anchors.}
\fontsize{8}{8}\selectfont
\centering
\begin{tabular}{c|c|c|c}
\toprule
         & Ours  & Multi-task & Full Finetune \\
\midrule
ResNet50 & -56.6 & -61.4      & -87.4         \\
VGG19    & -56.2 & -50.3      & -24.2         \\
\bottomrule
\end{tabular}
\label{tab:generalization_cls}
\end{table}

==> Tables/main_RD.tex <==
\begin{table*}[]

\caption{BD-rate comparison under different machine tasks with \textit{Swin} as anchor.}
\fontsize{8}{8}\selectfont
\centering
\begin{tabular}{c|c|c|c}
\toprule
                         & Classification & Detection & Segmentation \\
\midrule
%Base                             &        &        &              \\
Full Fine-tuning                    &  -87.4 &  -71.8  & -68.2  \\
Multi-task                       &  -61.4 &  -39.5  &  -39.6  \\
\midrule
ICCV'21~\cite{}                  &   -9.3 &   3.2   &  -1.4  \\
\midrule
TIC + SFT~\cite{}               &  -58.7 &  -23.9  &  -19.9  \\
TIC + Channel Selection~\cite{} &  -31.1 &   52.3  &   54.3  \\
Ours (TIC + Prompt)             &  -56.6 &  -51.9  &  -45.7  \\
\bottomrule
\end{tabular}
\label{table:main_RD}
\end{table*}

% \begin{table*}[]
% \label{table:main_RD}
% \centering
% \begin{tabular}{c|c|c|c|c|c|c|c}
% \toprule
%                   & Base & Full Finetune & Multi-task Full Finetune & Conv+SFT & Swin+SFT & Swin+Channel Selection & Ours (Swin + Prompt) \\
% \midrule
% Classification    &      &               &                          &          &          &                        &                      \\
% Detection         &      &               &                          &          &          &                        &                      \\
% Object Detection  &      &               &                          &          &          &                        &                     \\
% \bottomrule
% \end{tabular}
% \end{table*}

==> Tables/num_of_prompts.tex <==
\begin{table}[]
\caption{Ablation of the number of inserting prompts on the encoder. The anchor is our base codec (without any prompts) trained for human vision.}
\fontsize{8}{8}\selectfont
\centering
\begin{tabular}{c|c|c}
\toprule
                 & 16 (1/4 of iamge feature) & 64 \\
\midrule
Classification   &       -56.6            &              -56.7          \\
Object Detection &       \textcolor{red}{-51.9}            &              -50.9          \\
\bottomrule
\end{tabular}
\label{tab:num_prompt}
\end{table}

==> Tables/prompt_depth.tex <==
\begin{table}[]
\caption{Ablation of the depth of inserting prompts on the encoder. The anchor is the base codec trained for human vision.}
\fontsize{8}{8}\selectfont
\centering
\begin{tabular}{c|c|c|c|c}

\toprule
                 & 1 & 12 & 34 & 1234 \\
\midrule
Classification   & -54.1 & -56.6 & -41.5 & -56.6  \\
Object Detection & -38.0 & \textcolor{red}{-51.9} & -28.8 & \textcolor{red}{-42.2}  \\
\bottomrule
\end{tabular}
\label{tab:prompt_depth}
\end{table}

==> Tables/prompt_position.tex <==
\begin{table}[]
\caption{Ablation of insertion point of prompt tokens.}
\fontsize{8}{8}\selectfont
\centering
\begin{tabular}{c|c|c}
\toprule
                 & Every layer & Input only \\
\midrule
Classification   &  -56.6  &  -55.6   \\
Object Detection &  \textcolor{red}{-51.9}  &  -40.8   \\
\bottomrule
\end{tabular}
\label{tab:decoderside}
\end{table}

==> Tables/shared_window.tex <==
\begin{table}[]
\caption{Ablation of prompts sharing across windows.}
\fontsize{8}{8}\selectfont
\centering
\begin{tabular}{c|c|c}
\toprule
                 & Separate prompts  & Shared across windows \\
\midrule
Classification   &  -56.6  &  -47.7   \\
Object Detection &  \textcolor{red}{-51.9}  &  -33.9   \\
\bottomrule
\end{tabular}
\label{tab:sharedwindow}
\end{table}

==> Tables/with_or_without_prompts.tex <==
\begin{table}[h]

\fontsize{8}{8}\selectfont
\centering

\begin{tabular}{c|c}
\toprule
Encoder  & Decoder   \\
\midrule
IP-type  & TP-type   \\
IP-type  &      -    \\
      -  & TP-type   \\
\bottomrule
\end{tabular}
\label{table:wwoprompts}
\end{table}
